Decaffe: DHT Tree-Based Online Federated Fake News Detection

The proliferation of mobile social networks (MSNs) has transformed information dissemination, leading to increased reliance on these platforms for news consumption. However, this shift has been accompanied by the widespread propagation of fake news, posing significant challenges in terms of public panic, political influence, and the obscuring of truth. Traditional data processing pipelines for fake news detection in MSNs suffer from lengthy response times and poor scalability, failing to address the unique characteristics of news in MSNs, such as prompt propagation, large-scale quantity, and rapid evolution. This paper introduces a novel system named Decaffe - a DHT Tree-Based Online Federated Fake News Detection system. Decaffe leverages distributed hash table (DHT)-based aggregation trees for scalability and real-time detection, and it employs two model fine-tuning methods for adapting to mobile network dynamics. The system's structure includes a root, branches, and leaves for effective dissemination of a pre-trained model and ensemble-based aggregation of predictive results. Decaffe uniquely combines centralized server-based and decentralized serverless model fine-tuning approaches with personalized model fine-tuning, addressing the challenges of real-time detection, scalability, and adaptability in the dynamic environment of MSNs.

==> 6_impl.tex <==
\section{Implementation}
\label{sec: implementation}

We implemented {\systemNameAbbr} on top of Pastry \cite{rowstron2001pastry} (v.2.1) instead of implementing another distributed system core, and used Pytorch (v.1.11.1) as the imported \ac{ML} API in Pastry. 
Specifically, Pytorch is an open source \ac{ML} framework built on Python and has been widely used in \ac{ML} community. 
Pastry is used to implement the \ac{DHT}-baesd overlay network and routing protocol, which is similar to Kademlia \cite{maymounkov2002kademlia} and Chord \cite{stoica2003chord} that are widely adopted in numerous peer-to-peer  applications, such as BitTorrent \cite{BitTorrent}, Minerva \cite{bender2005minerva}, and YaCy \cite{yacy}. 



Three major modifications to Pastry and Pytorch are as follows:
1) We implemented the \ac{BERT} model training using \ac{PFL} loss function on the Pastry nodes and enabled model transmission and aggregation in centralized and decentralized on top of Pastry's routing protocol.
2) We implemented the majority voting ensemble on top of Pastry by adding predictive results aggregation on each Pastry node. 
3) We implemented communication status checker on top of Pastry so that a better model fine-tuning method can be determined by the root.
% \begin{enumerate}[leftmargin = 12mm]
%     \item We implemented the \ac{BERT} model training using \ac{PFL} loss function on the Pastry nodes and enabled model transmission and aggregation in centralized and decentralized on top of Pastry's routing protocol.
%     \item We implemented the majority voting ensemble on top of Pastry by adding predictive results aggregation on each Pastry node. 
%     \item We implemented communication status checker on top of Pastry so that a better model fine-tuning method can be determined by the root.
% \end{enumerate}



